How to Solve Contextual Goal-Oriented Problems with Offline Datasets?

We present a novel method, Contextual goal-Oriented Data Augmentation (CODA), which uses commonly available unlabeled trajectories and context-goal pairs to solve Contextual Goal-Oriented (CGO) problems. By carefully constructing an action-augmented MDP that is equivalent to the original MDP, CODA creates a fully labeled transition dataset under training contexts without additional approximation error. We conduct a novel theoretical analysis to demonstrate CODA's capability to solve CGO problems in the offline data setup. Empirical results also showcase the effectiveness of CODA, which outperforms other baseline methods across various context-goal relationships of CGO problem. This approach offers a promising direction to solving CGO problems using offline datasets.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}




\subsection{Linear MDP construction for augmented MDP}
Assume that the original contextual MDP is linear: $P(s'|s,a) = \langle \phi_P(s,a), \mu(s')\rangle$, and $r_c(s) = \langle \phi_R(c,s), \theta \rangle$, where $\phi_P \in \mathbb{R}_{d_p}$ and $\phi_R \in \mathbb{R}_{d_R}$.  We will show the construction of some new representation $\phi'_P(s,a)$ and $\phi'_R(s,a,c)$ such that the augmented MDP is also linear with extra dimensions.
\paragraph{For transitions.}
Let 
\begin{equation}
        \phi_{P}'(s,a)= 
\begin{cases}
    \begin{bmatrix}
    \phi_P(s,a)\\
    0
    \end{bmatrix},& \text{if } a \neq a^+ \\
    \begin{bmatrix}
    \mathbf{0},\\
    1
    \end{bmatrix},              & \text{otherwise;}
\end{cases}
\end{equation}
and 
\begin{equation}
    \mu_P'(s') =
\begin{cases} 
    \begin{bmatrix}
        \mu_P(s')\\
        0
    \end{bmatrix}
    \text{if } s \neq s^+\\
    \begin{bmatrix}
    \mathbf{0},\\
    1
    \end{bmatrix},              & \text{otherwise.}
\end{cases}
\end{equation}
We can verify the $\phi_P'$ and $\mu_P'$ satisfy the augmented MDP defined in Section~\ref{}.

% \textbf{For transitions}
% We want to extend $\phi_{P}$ to $\phi_{P}'$ and $\mu_{P}$ to $\mu_{P}'$ for $s,c,a^+$ and $s^+$, while maintaining linearity in the augmented MDP. If $\phi_{P}'$ and $\mu_{P}'$ have enough representation power, we can keep $\phi_{P}'(s,a) = \phi_P(s,a)$, $\mu_{P}'(s) = \mu_{P}(s)$, and solve $\phi_{P}'(s,a^+)$ and $\mu_{P}'(s^+)$. It turns out we need one extra dimension for $\phi_{P}'$ and $\mu_{P}'$:

% \begin{itemize}
%     \item Let $\phi_{P}'(s,a) = [\phi_{P}(s,a)^\top,0]$ and $\mu_{P}'(s') = [\mu_{P}(s')^\top,0]$.
%     \item Solve $\phi_{P}'(s,a^+)$: To satisfy that for all $s',s \in \mathcal{S}$, $\bar P (s'|s,a^+) = 0$, we just need an extra dimension for $\phi_{P}'(s,a^+)$ for all $s$ with norm = 1: $\phi_{P}'(s,a^+) = [\mathbf{0}^\top, 1]^\top$.

%     \item Given $\phi_P'(s,a^+)$, solve $\mu_{P}'(s^+)$: making $\mu_{P}'(s^+)$ parallel to $\phi'(s,a^+)$ with norm = 1, so we have $\bar P (s^+|s,a^+) = 1$.

    % \chingan{So maybe you meant: extend $\phi$ such that $\phi(s,a^+) = \mathbf{0}$ and define $\phi_P'(s,a) = [ \phi(s,a), \mathbbm{1}(a=a^+)]$
    
    % Similarly, 
    % extend
    % $\mu_{P}(s^+) = 0$ and define $\mu_P'(s) = [\mu_P(s), \mathbbm{1}(s=s^+)]^\top$.
    % }

% \end{itemize}


\paragraph{For reward.}
Let
\begin{equation}
        \phi_{R}'(c,s,a)= 
\begin{cases}
    \begin{bmatrix}
    \mathbf{0}\\
    0
    \end{bmatrix},& \text{if } a \neq a^+ \\
    \begin{bmatrix}
    2\phi_R(c,s),\\
    -1
    \end{bmatrix},              & \text{otherwise;}
\end{cases}
\end{equation}
and 
\begin{equation}
    \theta_R' = \begin{bmatrix}
    \theta_R\\
    1
    \end{bmatrix}.
\end{equation}
We can verify that the new $\phi_R'$ and $\theta_R'$ also satisfy the augmented MDP.

% For $a^+$, we create a new $\phi_{R}'(c,s, a^+) = [2\phi_{R}(c,s)^\top, -1]^\top$, let $\phi_{R}'(c,s,a) = [\mathbf{0}^\top, 0]$ for all other $a$, and let $\theta_R' = [\theta_R^\top, 1]^\top$. Then we have $\bar r_c(s,a^+) = \langle \phi_{R}'(c,s,a^+), \theta_{R}'\rangle$.

\aditya{So, here we are assuming that the reward map $\bar r_c(s,a)$ with values $\pm 1$ has a low-rank representation and the feature representation $\phi_R(c,s)$ for this decomposition is known?}
\chingan{Yes; it's only $\theta_R$ and $\mu_P$ are not known.}



\textbf{Joint representation for both transition and reward} Define $\phi(c,s,a) \in \mathbb{R}_{d_P+d_R+2}$ to be concatenation of $\phi_{P}'(s,a)$ and $\phi_{R}'(c,s,a)$: 

For $a \neq a^+$, $\phi(c,s,a) = \begin{bmatrix}
    \phi_{P}(s,a)\\
    \mathbf{0}
\end{bmatrix}$, which is only dependent on $\phi_P(s,a)$; 

For $a = a^+$, $\phi(c,s,a) = \begin{bmatrix}
    \mathbf{0}\\
    \bar{\phi}_R(c,s)
\end{bmatrix}$, where $\bar{\phi}_R(c,s) = \begin{bmatrix}
    1\\
    2\phi_R(c,s)\\
    -1
\end{bmatrix}$. In this case, $\phi(c,s,a)$ is only dependent on $\phi_R(c,s)$. 

Finally, we define $\theta = [\mathbf{0}^\top, \theta_R'^\top]^\top$ and $\mu(s) = [\mu_P'(s)^\top, \mathbf{0}^\top]^\top$. Then we finish the construction of the linear augmented MDP.
\chingan{Write down $P(s'|s,a)$ and $r(s,a,c)$ based on these def. Just to remind people what the augmented MDP achieves}

\chingan{\textcolor{red}{Augmented MDP is not  fully defined yet. }}

\chingan{Should talk about we modify the algorithm by only modifying the representation}

\subsection{Suboptimality for the augmented MDP}

Assume that we have a dataset containing $N$ transitions $\mathcal{D} = \{(s,a,s')\}$ that satisfies the compliance assumption in \cite{jin2021pessimism}, which we can always label as $r=0$. Also, assume we have another dataset with $N'$ context-goal samples: $\mathcal{D'}=\{(c, s)\}$ sampled from a joint distribution of contexts $p_c \times p_{s|c}$, where the support of $p_c$ is $\mathcal{C}$. We can add $N'$ fake transitions: $\{(s, a^+, s^+, r_c=1)\}$ from the joint context-goal dataset $\{(c, s)\}$, where $s \in \mathcal{S}_c$. Since the transition and reward kernel is not dependent on $h$, the new combined transition dataset (fully-labeled) $\mathcal{D}_{\text{aug}}$ still satisfies the compliance assumption. 
\chingan{Here we have a final horizon problem. For the theory, we need to make the embedding time dependent? Or I think we need an extra argument to show that optimal policy here is stationary.}
Let optimal policy $\pi_c^*$ be the optimal policy that maximizes the objective function (\ref{eq: kl_augobj}).

A direct adaptation of Theorem 4.4 in \cite{jin2021pessimism} gives the following lemma:
\chingan{Need to define how context $c$ is paired with $s,a$ }
\ying{data collection assumption}
\chingan{\textcolor{red}{NOTE: There're some important details on how s,a,c are paired and the horizon. This is not a direct adaption.}}
\begin{lemma}
\label{lemma: subopt}
Define $\Lambda=\sum_{i=1}^{N+N'}(\phi(c_i,s_i,a_i)\phi(c_i,s_i,a_i)^\top + \lambda I)$\footnote{For $N$ trajectory only data, since the representation is not dependent on $c$, we can just randomly label some $c$ for uniform notation.}, $\beta = c_0d(H_{\text{max}}+1)\sqrt{\zeta}$,   $\zeta = \log(2d(H_{\text{max}}+1))(N+N')/\xi), \lambda = 1, c_0 > 0$ is some absolute constant. Then w.p. at least $1-\xi$, for any $x\in \mathcal{S}$ and $c \in \mathcal{C}$, we have

\begin{equation}
 \text{SubOpt}(\text{Pess}(D_\text{aug}),x,c) \leq 2\beta \mathbb{E}_{\pi_c^*}[\sum_{h=1}^T(\phi(c,s_h,a_h)^\top\Lambda^{-1}\phi(c,s_h,a_h))^{1/2}|s_1 = x].   
\end{equation}
\end{lemma}
\ying{Can we say it is a direct adaptation without proof? $T$ is a random variable inside the expectation, but can be upper bounded by $H_{\text{max}}+1$. Treat it as a fixed horizon with $H_{\text{max}}+1$ but there's no uncertainty if the env terminates.}
% put everything inside \pi_c^* and then take it out, beta is the same.

Our construction of $\phi(c,s,a)$ is special in the sense that for $a \neq a^+$ it is only dependent on the original transition representation, and for $a=a^+$ it is only dependent on the original contextual reward representation. As a result, we can have another upper bound of the suboptimality as below:

\chingan{We need to have a notation for the augmented MDP's state and action spaces so we can point out where the trajectory lives}

\begin{lemma}
\label{lemma: decompose}
Define $\Lambda_P = \sum_{i=1}^N{\phi_P(s_i,a_i)\phi_P(s_i,a_i)^\top + \lambda I}$,

and $\Lambda_R = \sum_{i'=1}^{N'}{\bar{\phi}_R(c_{i'},s_{i'})\bar{\phi}_R(c_{i'},s_{i'})^\top + \lambda I}$.

For any trajectory $\{(c,s_h, a_h)_{h=1}^T\}$, we have
\begin{equation}
\begin{aligned}
&\sum_{h=1}^T(\phi(c,s_h,a_h)^\top\Lambda^{-1}\phi(c,s_h,a_h))^{1/2} \\
&\leq \sum_{h=1}^{T}[\mathbf{1}(a_h \neq a^+)(\phi_P(s_h,a_h)^\top\Lambda_P^{-1}\phi_P(s_h,a_h))^{1/2} + \mathbf{1}(a_h = a^+)(\bar{\phi}_R(c,s_h)^\top\Lambda^{-1}_R\bar{\phi}_R(c,s_h))^{1/2}].
\end{aligned}
\end{equation}
% (Proof: Sherman–Morrison formula)
\end{lemma}
See proof in Appendix~\ref{app:decomposition}.

\subsection{Sufficient coverage}
Notice that for an optimal policy, $a^+$ will appear at most once in the whole trajectory, which is only at the end of the trajectory.

\begin{theorem}
\label{theorem: coverage}
Suppose there exists an absolute constant $c^{\text{\textdagger}}$ s.t.

\begin{equation}
\begin{aligned}
&\mathcal{E}^{\text{\textdagger}}=\{\Lambda_P \geq I + c^{\text{\textdagger}}_0 N \mathbb{E}_{\pi^*_c}[\phi_P(s_h,a_h)\phi_P(s_h,a_h)^\top|s_1 = x, a_h \neq a^+, h\leq T] \\
&\text{and }\Lambda_R \geq I + c^{\text{\textdagger}}_1 N' \mathbb{E}_{\pi^*_c}[\bar{\phi}_R(c,s_h)\bar{\phi}_R(c, s_h)^\top|s_1 = x, a_h = a^+, h\leq T] \text{ for all $x\in\mathcal{S}$, $c \in \mathcal{C}$}\} 
\end{aligned}
\end{equation}
satisfies $P_{D_{\text{aug}}}(\mathcal{E}^{\text{\textdagger}} )\geq 1-\xi$. 

Then $\forall x \in\mathcal{S}$, $\forall c \in \mathcal{C}$,
\begin{equation}
\text{SubOpt}(\text{Pess}(D_{\text{aug}}), x,c) \leq c_1d^{3/2}\sqrt{\zeta}((H_{\text{max}}+1)^2N^{-1/2}+(H_{\text{max}}+1)N'^{-1/2})
\end{equation}   
\end{theorem}
w.p. at least $1-2\xi$, $d = \max(d_{\phi_P}, d_{\phi_R}+2)$.

See proof in Appendix~\ref{app:coverage} and a discussion about PDS in Appendix~\ref{app:pds}.

\aditya{What is the difference between this PEVI sketch and a PDS implementation to solve the same problem? I feel that the difference here is negligible? Similarly, would reward learning simply be the method where we do not have the uncertainty penalty in the reward during backward value iteration?}
\ying{The second coverage assumption only requires the labeled dataset covering the final goal-reaching step. In PDS, they first learn a ``pessimistic" reward function and then do PEVI.}
\paragraph{Remark} Our coverage assumption about the ``labeled" dataset requires that the context-goal dataset has sufficient coverage only where the optimal policy outputs $a^+$ given $c$. Thus it only requires ``positive" samples of context-goal pairs and no ``negative" context-goal pairs due to the pessimistic nature of the learning algorithm itself. The bound in~\cite{hu2023provable} (which requires learning an extra pessimistic reward function, see Appendix~\ref{app:pds}) also shares a similar form, but with a more strict coverage assumption on the labeled data, i.e. the labeled dataset should cover the whole trajectory:
\begin{equation}
\{\Lambda_{R'} \geq I + c^{\text{\textdagger}}_2 N' \mathbb{E}_{\pi^*_c}[\phi_R(c,s_h)\phi_R(c, s_h)^\top|s_1 = x, h\leq T],\forall x\}
\end{equation} 
due to a more general assumption of the multi-task setting. In our analysis, we utilize the specific goal-conditioned structure which requires a much weaker coverage assumption, and without the need to learn an extra reward function. 


==> new_proof.tex <==
% \clearpage
\section{\algo+PSPI: Theoretical Analysis}  \label{app:theory}



\paragraph{CGO Setup}

Let $\SS$, $\AA$ be the state and the action space, let $\CC$ be the context space. For a context $c\in\CC$, we let $G_c \subseteq \SS$ be its goal set. Let $P(s'|s,a)$ denote the transition kernel. 
We consider an infinite-horizon setting with discount $\gamma\in[0,1)$. 
Let $\Delta$ denote the space of distributions.
Given a policy $\pi:\SS\times\CC\to\Delta(\AA)$, we define its state-action value function (i.e. Q function) as 
\begin{align*}
    Q^\pi(s,c,a) \coloneqq \E_{\pi,P} \left[ \sum_{t=0}^T \gamma^t \one[s \in G_c ] | s_0 = s, a_0 = a  \right]
\end{align*}
where $T$ is the first time  the agent enters $G_c$ (a random variable dependent on $\pi$ and $P$).
We use $V^\pi(s,c) \coloneqq Q^\pi(s,c,\pi)$ to denote the value function $\pi$, 
where  we define the shorthand $f(\pi) \coloneqq \E_{a\sim \pi}[f(a)]$. 
By construction, we have $Q^\pi(s,c,a) \in [0,1]$. 

In the following, to simplify writing, we define $x=(s,c)$ and $\XX \coloneq \SS\times\mathcal{C}$. We use $G$ to denote the goal set, i.e., 
$G = \{ x \in \XX : x =(s,c), s \in G_c \}$.
We define the reward function 
$R(x) = \one[s \in G_c ] $ for $x=(s,c)$ and the transition kernel on $\XX$ accordingly as 
\begin{align*}
    P(x'|x,a) \coloneq P(s'|s,c,a) \one(c'=c)
\end{align*}
where we define the extended dyanmics
\begin{align*}
    P(s'|s,c,a) &= 
    \begin{cases}
        \mathbb{1}(s'=s^+),  & \text{if $s\in G_c$ or $s = s^+$}   \\
        P(s'|s,a), & \text{otherwise}
    \end{cases}
\end{align*}
where $x=(s,c)$ and $x'=(s',c')$. Notice the context does not change in the transition.
%
We would overload the notation and write $x$ in place of $(s,c)$, e.g., $Q^\pi(x,a) = Q^\pi(s,c,a)$.

We suppose there is an initial distribution $d_0\in\Delta(\XX)$\footnote{We can relax this assumption to use samples of $d_0$ easily}. In addition, we assume $x\sim d_0$ is not in $G$ almost surely. This is to simplify the presentation. If $x\in G$, the agent reaches goal immediately and no learning is needed.


We assume we're given with a policy class $\Pi:\{ \pi:\XX\to\Delta(\AA)\}$.
Our goal is to find a policy $\pi:\XX\to\AA$ to maximize the return (which roughly can be viewed as minimizing the time step to reaching the goal set $G$), i.e., $\max_\pi V^\pi(d_0) $. 
We use $\pi^*$ to denote the optimal policy and define $Q^* \coloneqq Q^{\pi^*}$, $V^* \coloneqq V^{\pi^*}$.  



% Directly solving $\MM$ with an offline RL algorithm is problematic, because \adith{ToDo} 

% Infinite horizon discounted MDP. Trajectory terminates upon reaching the goal and gets reward of 1. This is equal to staying in a zero-reward absorbing state after reaching the goal. 

%\chingan{See below for data assumption; probably should move it here}
%\adith{Yup. Just putting the placeholder here to fill in later. Reading the augmented MDP construction now.}

\paragraph{Data Assumption}
We suppose there is a distribution of transitions $\mu_{\dyn}(s,a,s') $ and a distribution of context-goal pairs $\mu_{\goal} (s,c)$, where $\mu_{\dyn}$ is consistent with the transition kernel of $\MM$ (i.e., $\mu_\dyn(s'|s,a) = P(s'|s,a)$) and $\mu_{\goal}(s|c)$ has a support within $G_c$.
%
We assume access to i.i.d. samples drawn from $\mu_d$ and $\mu_g$, giving the datasets 
\begin{align*}
    D_{\dyn} &= \{  (s_i,a_i,s_i') \sim \mu_{\dyn} \} \\
    D_{\goal} &= \{  (s_j,c_j) \sim \mu_{\goal} \} 
\end{align*}
% We denote $|D_{\dyn} | = N_\dyn$ and $|D_\goal| = $
% \aditya{Might be better to use different subscripts for the two? Can be misleading and suggest that the two $s_n$ observations are common to both datasets.}
In addition, we suppose we have access to $d_0$ (if not, we assume access to i.i.d. samples of $d_0$ and we can approximate $d_0$ by these samples as well, without changing the order of the main results).


\subsection{Augmented MDP}
\label{app:augmented_mdp}

% \paragraph{Augmented MDP}
% \begin{itemize}
%     \item $\bar{P}(s'|s^+,a) = \mathbb{1}(s'=s^+)$ for all $a$. 
%     \item For $s \neq s^+$, $\bar{P}(s'|s,a) = P(s'|s,a)$ for $a\neq a^+$, and $\bar{P}(s'|s,a^+) = \mathbb{1}(s'=s^+)$.
%     \item $\bar r_c(s,a^+) = 1$ when $s \in \mathcal{G}_c$ and $-1$ when $s \notin \mathcal{G}_c$.
%     \item For  $a \ne a^+$, $\bar r_c(s,a) = 0$. 
% \end{itemize}

We define an augmented MDP to reformulate the CGO problem. 
We introduce a fictitious state $s^+$ and a fictitious action $a^+$.
Define $\bar{\SS} = \SS \bigcup \{ s^+ \}$ and $\bar{\AA} = \AA \bigcup \{ a^+ \}$. In addition, we define $\XX^+ = \{ (s^+,c) | c \in \CC \}$ and $\bar{\XX} = \XX \bigcup \XX^+$. Notice $G \bigcap \XX^+ = \emptyset$.

The augmented MDP has state space $\bar{\XX}$ and action space $\bar{A}$.
We define its dynamics and reward as follows: For $x=(s,c)\in\bar{X}$, 
\begin{align*}
    \bar{P}(x'|x,a) &\coloneq \bar{P}(s'|s,a) \one(c'=c )\\
    \bar{R}(x,a) &\coloneq
    \begin{cases}
        \one( s\in G_c), %- \one( s\notin G_c) 
        &\text{if $a=a+$} \\
        0 , &\text{otherwise} 
    \end{cases}
\end{align*}
where the transition of the $\bar{S}$ part is defined as 
\begin{align*}
    \bar{P}(s'|s,a) &= 
    \begin{cases}
        \mathbb{1}(s'=s^+),  & \text{if $s=s^+$ or $a=a^+$}   \\
        P(s'|s,a), & \text{otherwise}
    \end{cases}
\end{align*}



%
The augmented MDP is denoted as $\overline{\MM} \coloneq (\bar\XX, \bar\AA, \bar{R}, \bar{P}, \gamma)$. 
For policy and value functions defined in the original MDP, we define their extensions on the augmented MDP, which has larger state and action spaces.
%
Given $\pi: \XX \to \Delta(\AA)$, we define its extension $\bar{\pi}:\bar\XX\to\Delta(\bar\AA)$ as
\begin{align} \label{eq:policy extension}
    \bar{\pi}(a|x) = 
    \begin{cases}
        \pi(a|x), & \text{$x\notin G$}\\
        a^+, & \text{otherwise}
    \end{cases}
\end{align}
Given $f:\XX\times\AA \to [0,1] $ (e.g. the Q function) and $ g:\XX \to [0,1]$, we define an extension $\bar{f}_g:\bar\XX\times\bar\AA\to[0,1]$ as
\begin{align} \label{eq:value extension}
    \bar{f_g}(x,a) = 
    \begin{cases}
        g(x), & \text{$a= a^+$, $x\notin \XX^+$}\\
        0, & \text{$x \in \XX^+$}\\
        f(x,a), & \text{otherwise}
    \end{cases}
\end{align}
% \aditya{$f$ needs to be defined over $\XX \times \AA$. This step would extend the definition from $\XX \times \AA$ to $\XX^+ \times \bar \AA$.}

For a policy $\bar{\pi}: \bar\XX \to \bar\AA$, we define the Q function for the augmented MDP as 
\begin{align*}
    \bar{Q}^{\bar{\pi}}(x,a) \coloneqq \E_{\bar\pi,\bar{P}} \left[ \sum_{t=0}^\infty \gamma^t \bar{R}(x,a) | x_0 = x, a_0 = a  \right]
\end{align*}
Notice that we don't have a reaching time random variable $T$ in this definition; instead the agent would enter an absorbing state $s^+$ after taking $a^+$ in the augmented MDP. We can define similarly $\bar{V}^{\bar\pi}(s) \coloneq \bar{Q}^{\bar{\pi}}(x,\bar{\pi})$.


\begin{remark}
\chingan{corrected}
Let $\bar{Q}^\pi_R$ be the extension of $Q^\pi$ based on $R$.
We have, for $x \notin G$, $\bar{Q}^\pi_{{R}} (x,a) = \bar{Q}^{\bar{\pi}} (x,a)$ $\forall a \in \bar\AA$, and for $x \in G$, $\bar{Q}^\pi_{{R}} (x,a) =  \bar{Q}^{\bar{\pi}} (x,a^+) = 1$, $\forall a\in\bar\AA$.
\end{remark}

By the construction of the augmented MDP, it is obvious that the following is true.
\begin{lemma} \label{lm:equivalence}
    Given $\pi:\XX\to\Delta(\AA)$, let $\bar\pi$ be its extension.
    For any $h:\XX\times\AA\to \R$, it holds
    \begin{align*}
        \E_{\pi,P} \left[ \sum_{t=0}^T \gamma^t h(x,a) \right] = \E_{\bar\pi,\bar{P}} \left[ \sum_{t=0}^\infty \gamma^t \tilde{h}^\pi(x,a) |  x \notin \XX^+ \right]
    \end{align*}
    where $T$ is the goal-reaching time (random variable) and we define $\tilde{h}^\pi(x,a^+)=h(x,\pi)$. 
\end{lemma}
% \chingan{Relate to $d^\pi$}


%\adith{Nitpick: Off-by-one error? The time-step $T$ that a policy, after landing in $s \in G_c$, takes any action and gets reward of $1$ should be the same time-step that the augmented policy takes $a^+$ action getting the reward of $1$, so that the discounting works out ok. However, the original $Q^\pi(s,c,a)$ definition may need the summation to go to $T+1$ because it is only on the timestep after entering $G_c$ that the policy should receive the reward in the original MDP? }


We can relate the value functions between the two MDPs. 
\begin{proposition} \label{lm:Q equivalence}
\chingan{corrected}
For a policy $\pi:\SS\to\Delta(\AA)$, let $\bar{\pi}$ be its extension (defined above). We have for all $x\in\XX$, $a\in\AA$,  
\begin{align*}
    Q^\pi(x,a) &\geq \bar{Q}^{\bar{\pi}}(x,a)\\
    V^\pi(x) &= \bar{V}^{\bar{\pi}}(x)
\end{align*}
Conversely, for a policy $\xi:\bar\XX\to\Delta(\bar{\AA})$, define its restriction $\underline{\xi}$ on $\XX$ and $\AA$ by translating probability of $\xi$ originally on $a^+$ to be uniform over $\AA$.  Then we have for all $s\in\SS$, $a\in\AA$
\begin{align*}
    Q^{\underline\xi}(x,a) &\geq  \bar{Q}^{\xi}(x,a)\\
    V^{\underline\xi}(x) &\geq  \bar{V}^{\xi}(x)
\end{align*}
\end{proposition}
\begin{proof}
The first direction follows from \cref{lm:equivalence}. For the latter, whenever $\xi$ takes $a^+$ at some $x\notin G$, it has $\bar{V}^\xi(x) = 0$ but $\bar{V}^{\underline\xi}(x)\geq 0$ since there is no negative reward in the original MDP.  By performing a telescoping argument, we can derive the second claim.
\end{proof}



By this lemma, we know the extension of $\pi^*$ (i.e., $\bar{\pi}^*$) is also optimal to the augmented MDP and $V^*(x) = \bar{V}^*(x)$ for $x\in\XX$. Furthermore, we have a reduction that we can solve for the optimal policy in the original MDP by the solving augmented MDP, since 
\begin{align*}
    V^{\underline\xi}(d_0) - V^*(d_0) \leq V^{\xi}(d_0) - \bar{V}^*(d_0)
\end{align*}
for all $\xi:\bar{\XX}\to\Delta(\AA)$. 
In particular, 
\begin{align}
    \text{Regret}(\pi) \coloneq  V^{\pi}(d_0) - V^*(d_0) = V^{\bar\pi}(d_0) - \bar{V}^*(d_0) \eqcolon \overline{\text{Regret}}(\bar\pi)
\end{align}


Since the augmented MDP replaces the random reaching time construction with an absorbing-state version, the Q function $\bar{Q}^{\bar\pi}$ of the extended policy $\bar\pi$ satisfies the Bellman equation
\begin{align}
    \bar{Q}^{\bar\pi}(x,a) 
    &= \bar{R}(x,a) + \gamma \mathbb{E}_{x'\sim \bar{P}(\cdot|x,a)} [ \bar{Q}^{\pi}(x',\bar{\pi}) ] \nonumber\\
    &\eqcolon \bar{\TT}^\pi \bar{Q}^{\pi}(x,a)    \label{eq:augment_BE}
\end{align}
For $x\in\XX$ and $a\in\AA$, we show how the above equation can be rewritten in $Q^\pi$ and $R$. 
% 
% We have for $x\in\XX$ and $a\in\AA$, by \cref{lm:max Q and r},
% \begin{align*}
%     Q^{\pi}(x,a) 
%     &= \bar{Q}^{\bar\pi}(x,a) = R(x) + \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))  ]    
% \end{align*}
% where $R(x) = R(s,c)$
% For $x\in \XX^+$, $ \bar{Q}^{\bar\pi}(x,a) = 0$.
\begin{proposition} \label{eq:Bellman eqation mod}
% \chingan{corrected: should be $0$ instead of $R(x)$}
For $x\in\XX$ and $a\in\AA$,
    \begin{align*}
    \bar{Q}^{\bar\pi}(x,a) = 0 + \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))  ]    
\end{align*}
For $a = a^+$, $\bar{Q}^{\bar\pi}(x,a^+) = \bar{R}(x,a^+) = R(x)$.
For $x \in \XX^+$, $\bar{Q}^{\bar\pi}(x,a) = 0$.
\end{proposition}



\begin{proof}
    The proof follows from \cref{lm:max Q and r} and the definition of $\bar{P}$.
\end{proof}
\begin{lemma} \label{lm:max Q and r}
For $x\in\XX$, $\bar{Q}^{\bar\pi}(x,\bar{\pi})  = \max(R(x),Q^{\pi}(x, \pi))$
\end{lemma}
\begin{proof}
     For $x\in\XX$,
\begin{align*}
     \bar{Q}^{\bar\pi}(x,\bar{\pi}) 
     &= 
     \begin{cases}
         \bar{Q}^{\bar\pi}(x, a^+), \quad &\text{if $x\in G$}\\
         \bar{Q}^{\bar\pi}(x, \pi), \quad &\text{otherwise}
     \end{cases} &\text{(Because of definition of $\bar{\pi}$) }
     \\
     &= 
     \begin{cases}
         \bar{Q}^{\bar\pi}(x, a^+), \quad &\text{if $x\in G$}\\
         Q^{\pi}(x, \pi), \quad &\text{otherwise}
     \end{cases}    \qquad &\text{(Because of \cref{lm:Q equivalence}) }
     \\
     &=
     \begin{cases}
         \bar{R}(x,a^+ ), \quad &\text{if $x\in G$}\\
         Q^{\pi}(x, \pi), \quad &\text{otherwise}
     \end{cases}    \qquad &\text{(Definition of augmented MDP) }
  \\
  &=
     \begin{cases}
         R(x), \quad &\text{if $x\in G$}\\
         Q^{\pi}(x, \pi), \quad &\text{otherwise}
     \end{cases}  \\
     % &= \max(\bar{R}(x,a^+ ),Q^{\pi}(x, \pi))\\
     &= \max(R(x),Q^{\pi}(x, \pi))
\end{align*}
where in the last step we use $\bar{R}(x)=1$ for $x\in G$ and $\bar{R}(x) = 0$ otherwise.
\end{proof}




% We also define the reframed Bellman backup operator
% \begin{align*}
%     \KK^\pi \bar{f}_g (x,a) \coloneq R(x) + \gamma \E_{x'\sim P(\cdot|x,a)} [ \max(g(x'),f(x',\pi)) ]
% \end{align*}
% We summarize the above as follows
% \begin{proposition}
% \chingan{this summarization is wrong}
% For $x\in\XX$ and $a\in\AA$
% \begin{align}
%     Q^\pi(x,a) = \TT^\pi Q^\pi(x,a) =  \KK^\pi \bar{Q}_R^\pi (x,a)
% \end{align}    
% \end{proposition}




\subsection{Function Approximator Assumptions}

% \chingan{We need to make this assumption to be based on the augmented mdp, at least we need the absorbing state to make the writing simpler.}
% \chingan{Probably we go with perfect realizability for now. There're some minor but annoying technical details to handle the error. }
We assume a policy class $\Pi = \{ \pi: \XX \to \Delta(\AA)\}$.
%
We also assume  access to a function class $\FF = \{ f: \XX\times\AA \to [0,1]\}$ and a function class $\GG = \{ g: \XX \to [0,1]\}$. We can think of them as approximator for the Q function and the reward function of the original MDP. 


% Let $d^\pi(x,a) = (1-\gamma)\sum_{t=0}^\infty \gamma^t d_t^\pi(x,a)$, where $d_t^\pi$ is the state-action distribution of running policy $\pi$ in the MDP $\MM = (\XX,\AA,r,P,\gamma)$. 
%
% Let $\Omega \coloneq \{ d^\pi : \pi \in \Pi \} $ denote the set of all possible average state-action distributions. 

Define a zero-reward Bellman backup operator $\TT^\pi$ with respect to $P(s'|s,a)$
\begin{align*}
    \TT^\pi f (x,a) \coloneq \gamma \E_{x'\sim P_0(\cdot|x,a)} [ f(x',\pi) ]
\end{align*}
where $P_0(x'|x,a) \coloneq P(s'|s,a) \one(c'=c)$. Note this definition is different from the one with absorbing state $s^+$ in \cref{sec:notation}. \chingan{updated}


% We make the following realizability and completeness assumptions. 
% \begin{assumption}[Realizability] \label{as:realizability}
% We assume for any $ \pi \in \Pi$, $Q^\pi\in\FF$ and $R \in\GG$.
% \end{assumption}

% \begin{assumption}[Completeness] \label{as:completeness}
% We assume   
% \begin{itemize}       
%     \item For any $f\in\FF$ and $g\in\GG$, $\max(g(x),f(x,\pi)) \in \FF$ 
%    \item For any $f\in\FF$, $\pi \in \Pi$, $\TT^\pi f (x,a) \in \FF$
%    \end{itemize}
% \end{assumption}

% \chingan{working...}
\begin{proposition}[Realizability] \label{lm:realizability}
By \cref{as:realizability} and \cref{as:completeness}, there is $f\in\FF$ and $g\in\GG$ such that $\bar{Q}^{\bar{\pi}} = \bar{f}_g$. 
\end{proposition}
\begin{proof}
By \cref{as:completeness}, there is $h\in\FF$ such that $h(x,a) =  \max(R(x),Q^{\pi}(x, a)) $.
By \cref{eq:Bellman eqation mod}, we have for $x\in\XX$, $a\neq a^+$
\begin{align*}
    \bar{Q}^{\bar\pi}(x,a) 
    &= 0 + \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))  ]    \\
    &= 0 + \gamma \E_{x'\sim P_0(\cdot|x,a)} [  h(x,\pi)  ]  \\
    &= \TT^\pi h \in \FF
\end{align*}
For $a=a^*$, we have
$ \bar{Q}^{\bar\pi}(x,a^*) = \bar{R}(x,a^+) = R(x) \in \GG$. 
Finally $\bar{Q}^{\bar\pi}(x^+,a) = 0$ for $x^+ \in \XX^+$. 
%
Therefore, $\bar{Q}^{\bar{\pi}} = \bar{f}_g$ for some $f\in\FF$ and $g\in\GG$.
\end{proof}

% \chingan{Ah. We need to define $d^\pi$ with the absorbing. }
% Let $d^\pi(x,a) = (1-\gamma)\sum_{t=0}^\infty \gamma^t d_t^\pi(x,a)$, where $d_t^\pi$ is the state-action distribution of running policy $\pi$ in the MDP $\MM = (\XX,\AA,r,P,\gamma)$. 
% %
% Let $\Omega \coloneq \{ d^\pi : \pi \in \Pi \} $ denote the set of all possible average state-action distributions. Define the Bellman backup operator $\TT^\pi$ as 
% \begin{align*}
%     \TT^\pi f (x,a) \coloneq R(x) + \gamma \E_{x'\sim P(\cdot|x,a)} [ f(x',\pi) ]
% \end{align*}


% We make the following realizability and completeness assumptions. 
% \begin{assumption}[Approximate Realizability] \label{as:realizability}
% We assume for any $ \pi \in \Pi$ % $Q^\pi\in\FF$ and $r\in\GG$.
%    \begin{itemize}
%        \item  $ \min_{g\in\GG} \sup_{\nu \in \Omega} \E_{x,a\sim \nu} [ | g(x) - R(x)|^2  ] \leq \epsilon_{\FF,\GG}$
%        \item $ \min_{f\in\FF} \sup_{\nu \in \Omega} \E_{x,a\sim \nu} [ | f(x,a) - \TT^\pi f(x,a)|^2  ] \leq \epsilon_{\FF,\GG}$
%    \end{itemize}
% \end{assumption}

% \begin{assumption}[Approximate Completeness] \label{as:completeness}
% We assume   
% \begin{itemize}       
%     \item For any $f\in\FF$ and $g\in\GG$, $\max(g(x),f(x,\pi)) \in \FF$ 
%    \item For any $f\in\FF$, $\pi \in \Pi$,
%  $ \min_{f'\in\FF}  \E_{x,a\sim \mu} [ | f'(x,a) - \TT^\pi f (x,a)] |^2  ] \leq \epsilon_{\FF,\GG}$
%    \end{itemize}
% where $\mu$ is the data distribution \chingan{define this later on.}
% \end{assumption}




We define the generalized concentrability coefficients~\citep{xie2021bellman}
\begin{definition}
Given two distributions $\nu$ and $\mu$, we define the generalized concentrability coefficients:
    \begin{align*}
        \mathfrak{C}_{\dyn}(\nu, \mu, \FF, \pi) &\coloneq \max_{f,f'\in\FF} \frac{\| f - \TT^\pi f' \|_\nu^2}{ \| f - \TT^\pi f' \|_\mu^2}\\
        \mathfrak{C}_{\goal}(\nu, \mu, \GG, \pi) &\coloneq \max_{g\in\GG} \frac{\| g-r \|_\nu^2}{ \| g-r \|_\mu^2}
    \end{align*}
where $\|h \|_\mu^2 \coloneq \E_{x\sim\mu}[ h(x)^2]$.
\end{definition}

% \begin{remark}
%     An alternate (and more direct) completeness assumption can be stated as: 
% For any $f\in\FF$ and any $g\in\GG$, $\pi \in \Pi$,$\KK^\pi \bar{f}_g \in \FF$. 
%  \cref{as:completeness} is a sufficient condition to this. When using version, we would modify the definition of $\mathfrak{C}_{\dyn}$ accordingly as
%  \begin{align*}
%     \mathfrak{C}_{\dyn}(\nu, \mu, \FF, \GG, \pi) &\coloneq \max_{f\in\FF,g\in\GG} \frac{\| \bar{f}_g - \KK^\pi \bar{f}_g \|_\nu^2}{ \| \bar{f}_g - \KK^\pi \bar{f}_g \|_\mu^2}
%     \end{align*}
% \end{remark}
% \begin{remark}
%     An alternate (and more direct) $\epsilon$-completeness assumption can be stated as: 
% For any $f\in\FF$ and any $g\in\GG$, $\pi \in \Pi$,
%  $ \min_{f'\in\FF}  \E_{x,a\sim \mu} [ | f'(x,a) -  \KK^\pi \bar{f}_g |^2  ] \leq \epsilon$. 
%  \cref{as:completeness} is a sufficient condition to this. When using version, we would modify the definition of $\mathfrak{C}_{\dyn}$ according to be based on $\max( g(x'), f(x',\pi))$.
% \end{remark}

\subsection{Algorithm}

Our algorithm is based on the idea of reduction, which turns the offline CGO problem into an standard offline RL problem in the augmented MDP. To this end, we define the augmented datasets based on $D_{\dyn}$ and $D_{\goal}$.
\begin{align*}
    \bar{D}_\dyn &= \{ (x_n,a_n,r_n,x_n') |  r_n=0, x_n = (s_i, c_j), x_n' = (s_i', c_j), a_n = a_i, (s_i,a_i,s_i') \in D_\dyn, (\cdot, c_j) \in D_\goal \}\\
    \bar{D}_\goal &= \{ (x_n, a^+,r_n, x_n^+) | r_n=1, x_n = (s_n, c_n), x_n^+ = (s^+, c_n), (s_n, c_n)\in D_\goal  \}
\end{align*}
That is, $\bar{D}_\dyn \sim \mu_\dyn(s,a,s') \mu_\goal(c)$ and $\bar{D}_\goal \sim \mu_\goal(c,s) \one(a=a^+)\one(s'=s^+) $.
With abuse of notation, we write $\mu_\dyn(x,a,x') = \mu_\dyn(s,a,s') \mu_\goal(c)$ and $\mu_\goal(x,a,x') = \mu_\goal(c,s) \one(a=a^+)\one(s'=s^+)$.
%
These two datasets have the standard tuple format, so we can run offline RL on $\bar{D}_\dyn \bigcup \bar{D}_\goal$.

Here we showcase how this can be done with PSPI in \cite{xie2021bellman}; we can follow a similar logic to apply this to other algorithms like ATAC \cite{cheng2022adversarially}, etc.

% \chingan{Need to update the presentation a bit.}
\paragraph{Background: PSPI}
We consider the information theoretical version of PSPI. It can be summarized as follows: 
For an MDP $(\XX,\AA,R,P,\gamma)$, given a tuple dataset $D =\{ (x,a,r,x')\}$, a policy class $\Pi$, and a value class $\FF$, it finds the policy through solving the two-player game:
\begin{align}\label{eq:pspi_app}
    \max_{\pi\in\Pi}  \min_{f\in\FF} \quad f(d_0, \pi) \qquad \text{s.t.}  \qquad 
    \ell(f,f;\pi,D) - \min_{f'\in\FF} \ell(f',f;\pi,D) \leq \epsilon_b
\end{align}
where $ \ell(f,f';\pi,D) \coloneq \frac{1}{|D|} \sum_{(x,a,r,x')\in D}  (f(x,a) - r - f'(x',\pi))^2
$ is the temporal difference error on the data.
The term $\ell(f,f;\pi,D) - \min_{f'} \ell(f',f;\pi,D)$ in the constraint is an empirical estimation of the Bellman error on $f$ with respect to $\pi$ on the data distribution $\mu$, i.e. $ \E_{x,a\sim\mu} [(f(x,a) - \TT^\pi f(x,a))^2]$. It constrains the Bellman error to be small as we know $ \E_{x,a\sim\mu} [(Q^\pi(x,a) - \TT^\pi Q^\pi(x,a))^2] = 0$.
%
% \chingan{Issue: here I use $s$. Should I use $x$?}\aditya{I think we can replace $\SS$ with $\XX$ here. }


Below we show how to run PSPI to solve the augmented MDP with offline dataset $\bar{D}_\dyn \bigcup \bar{D}_\goal$.
To this end, we extend the policy class from $\Pi$ to $\bar{\Pi}$ based on the extension in \eqref{eq:policy extension}, and the value class from $\FF$ to $\bar{\FF}_\GG$ using the function class $\GG$ following \eqref{eq:value extension}.
%
One natural attempt is to implement \eqref{eq:pspi} with the extended policy and value classes  $\bar{\Pi}$ and $\bar{\FF}$ and $\bar D = \bar{D}_\dyn  \bigcup \bar{D}_\goal$.
%
This would lead to the two player game: 
\begin{align}\label{eq:pspi (augemnted)}
    \max_{\bar\pi\in\bar\Pi} \min_{\bar{f}_g\in\bar\FF_\GG} \quad 
    \bar{f}_g (d_0, \bar\pi) \qquad \text{s.t.}  \qquad 
    \ell( \bar{f}_g, \bar{f}_g ;\bar\pi,\bar{D}) - \min_{\bar{f}_{g'}'\in\bar\FF_\GG} \ell(\bar{f}_{g'}',\bar{f}_g;\bar\pi,\bar{D}) \leq \epsilon_b
\end{align}
However, \eqref{eq:pspi (augemnted)} is not a well defined algorithm, because its usage of the extended policy $\bar\pi$ in the constraint requires knowledge of $G$, which is unknown to the agent. 



Fortunately, we show that \eqref{eq:pspi (augemnted)} can be slightly modified so that the implementation does not actually require knowing $G$. 
%
Here we use a property (\cref{eq:Bellman eqation mod}) that the Bellman equation of the augmented MDP: 
\begin{align*}
    \bar{Q}^{\bar\pi}(x,a) 
    &= \bar{R}(x,a) + \gamma \mathbb{E}_{x'\sim \bar{P}(\cdot|x,a)} [ \bar{Q}^{\pi}(x',\bar{\pi}) ] \\
    &= 0 + \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))  ]    
    % &= Q^\pi(x,a)
\end{align*}
for $x\in\XX$ and $a\neq a^+$, and  $    \bar{Q}^{\bar\pi}(x,a) = 1 $ for $x\in G$ and $a=a^+$.

% For $x\in\XX$
% \begin{align}
%     \bar{Q}^{\bar\pi}(x,\bar{\pi}) = \max(R(x'),Q^{\pi}(x', \pi)) 
% \end{align}
% Note that $\bar{Q}^{\pi}(x,a) = Q_r^\pi(x,a)$, i.e., \chingan{true?}
% \begin{align*}
%     \bar{Q}^{\pi}(x,a) =
%     \begin{cases}
%         R(x), & \text{if } x\in G\\
%         0,  &\text{if } x\in X^+ \\
%         Q^\pi(x,a), &\text{otherwise}
%     \end{cases}
% \end{align*}


We apply these two equalities  to $D_\dyn$ and $D_\goal$ to construct our Bellman error estimates. 
Let $\phi(\bar{Q}^{\bar\pi}(x)) \coloneq  \max(R(x),Q^{\pi}(x, \pi))$. We can rewrite the squared Bellman error on these two data distributions using the Bellman backup defined on the augmented MDP (see eq.\ref{eq:augment_BE}) as below:
\begin{align*}
 \E_{x,a\sim\mu_\dyn} [(\bar{Q}^{\bar\pi}(x,a) - \bar\TT^{\bar\pi} \bar{Q}^{\bar\pi}(x,a))^2] 
 &= 
 \E_{x,a\sim\mu_\dyn} [(\bar{Q}^{\bar\pi}(x,a) - 0 - \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [ \phi(\bar{Q}^{\bar\pi})(x',\pi) ] )^2]
\end{align*}
\begin{align*}
 \E_{x,a\sim\mu_\goal} [(\bar{Q}^{\bar\pi}(x,a) - \bar\TT^{\bar\pi} \bar{Q}^{\bar\pi}(x,a))^2] 
 &= \E_{x,a\sim\mu_\goal} [(\bar{Q}^{\bar\pi}(x,a^+) - 1)^2] 
\end{align*}

% \chingan{Need to update}
% Recall that $\bar{Q}^{\bar\pi} = \bar{Q}_{R}^{\pi}$, where by the extension rule
% \begin{align*}% \label{eq:value extension}
%     \bar{Q}_R^{\pi}(x,a) = 
%     \begin{cases}
%         R(x), & \text{$a= a^+$}\\
%         0, & \text{$x \in \XX^+$}\\
%         Q^\pi(x,a), & \text{otherwise}
%     \end{cases}
% \end{align*}
% Therefore, using $f(x,a)$ as an approximate of $Q^\pi(x,a)$ and $g(x)$ as an approximate of $R(x)$, 
\chingan{Updated}
We can construct an approximator $\bar{f}_g(x,a)$ for $\bar{Q}^{\bar\pi}(x,a)$. 
Substituting the estimator $\bar{f}_g(x,a)$  for $\bar{Q}^{\bar\pi}(x,a)$ in the squared Bellman errors above and approximating them by finite samples, we derive the empirical losses below. 

% That is, we wish to approximate on $D_\dyn$
% \begin{align*}
%   &   \frac{1}{|D_\dyn|} \sum_{(x,a,r,x')\in D_\dyn} ( \bar{f}_g(x,a) - R(x) - \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(g(x'), f(x', \pi))  ]   )^2\\
%  &=   \frac{1}{|D_\dyn|} \sum_{(x,a,r,x')\in D_\dyn} ( f(x,a) - 0 -  \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(g(x'), f(x', \pi))  ]   )^2
% \end{align*}
% We approximate $\bar{Q}^{\bar\pi} $ with $f_g$ and $r$ with $g$.
% And on $D_\goal$, 
% \begin{align*}
%   &   \frac{1}{|D_\goal|} \sum_{(x,a,r,x')\in D_\dyn} ( \bar{f}_g(x,a) - R(x)    )^2 =   \frac{1}{|D_\goal|} \sum_{(x,a,r,x')\in D_\dyn} ( g(x) -1   )^2
% \end{align*}
% \chingan{Turn this into a lemma?}
% \begin{lemma}\label{eq:loss simplification}
%         Blah
% \end{lemma} 
\begin{align} \label{eq:empirical losses}
    \ell_\dyn(\bar{f}_g,\bar{f}'_{g'}; \bar\pi) &\coloneq \frac{1}{|D_\dyn|} \sum_{(x,a,r,x')\in D_\dyn} ( f(x,a) - \gamma    \max(g'(x'), f'(x', \pi))    )^2\\
    \ell_\goal(\bar{f}_g) &\coloneq \frac{1}{|D_\goal|} \sum_{(x,a,r,x')\in D_\dyn} ( g(x) -1   )^2
\end{align}
where we use $\phi(\bar{f}_g)(x,a) =  \max(g(x), f(x,a)) $ and for $x\notin\XX^+$, $\bar{f}_g(x,a) = f(x,a) \one(a\neq a^+) + g(x) \one(a=a^+)$. 
% \chingan{Relate this to our IQL implementation}

Using this loss, we define the two-player game of PSPI for the augmented MDP: 
\begin{align}\label{eq:pspi (augemnted) (real)}
    &\max_{\bar\pi\in\bar\Pi} \min_{\bar{f}_g\in\bar\FF} \bar{f}_g (d_0, \bar\pi) \qquad \\
    &\text{s.t.} \nonumber \\
    &\ell_\dyn( \bar{f}_g, \bar{f}_g ;\bar\pi) - \min_{\bar{f}_{g'}'\in\bar\FF} \nonumber \ell_\dyn(\bar{f}_{g'}',\bar{f}_g;\bar\pi) \leq \epsilon_\dyn \\
    &\ell_\goal (\bar{f}_g) \leq  0 \nonumber
\end{align}
Notice $\bar{f}_g (d_0, \bar\pi) = f(d_0, \pi)$. Therefore, this problem can be solved using samples from $D$ without knowing $G$.


\subsection{Analysis}


\paragraph{Covering number}
We first define the covering number on the function classes $\FF$, $\GG$, and $\Pi$. 
For $\FF$ and $\GG$, we use the $L_\infty$ metric. We use $\NN_\infty(\FF,\epsilon)$ and $\NN_\infty(\GG,\epsilon)$ to denote the their $\epsilon$-covering numbers. 
%
For $\Pi$, we use the $L_\infty$-$L_1$ metric, i.e., $\| \pi_1 -  \pi_2\|_{\infty,1} \coloneq  \sup_{x\in\XX} \| \pi_1(\cdot|s) - \pi_2(\cdot|s) \|_1$. We use $\NN_{\infty,1}(\Pi,\epsilon)$ to denote its $\epsilon$-covering number. 

\paragraph{High-probability Events}
% \chingan{Aditya please double check}

First, we show $\bar{Q}^{\bar{\pi}}$ has small empirical errors.
% \begin{lemma}\label{lm:Qpi in the set}
% Denote, for each $\pi\in\Pi$,
% \begin{align*}
%     \tilde{f}_g^\pi = \arg\min_{f\in\FF,g\in\GG} \sup_{\nu\in\Omega} \| f(s,a) - \gamma \E_{x'\sim P(\cdot|x,a)} [ \max( g(x'), f(x',\pi)  ] \|_{\nu}^2
% \end{align*} \chingan{Change definition to be realizability}
% With probability at least $1-\delta$, it holds for all $\pi\in\Pi$,
% \begin{align*}
%         &\ell_\dyn( \tilde{f}_g^\pi, \tilde{f}_g^\pi ;\bar\pi) - \min_{\bar{f}_{g'}'\in\bar\FF} \ell_\dyn(\bar{f}_{g'}',\tilde{f}_g^\pi;\bar\pi) \leq \epsilon_\dyn\\
%     &\ell_\goal (\tilde{f}_g^\pi) \leq 0 
% \end{align*}
% where 
% \begin{align*}
%     &\epsilon_\dyn = O\left( {\frac{\log \frac{ \NN_\infty(\FF, \frac{1}{|D_\dyn|}) \NN_\infty(\GG, \frac{1}{|D_\dyn|})\NN_{\infty,1}(\Pi,\frac{1}{|D_\dyn|})}{\delta} }{|D_\dyn|}} + {\epsilon_{\FF,\GG}}  \right)
%     % &\epsilon_\goal = O\left( \sqrt{\frac{\log \frac{\NN_\infty(\GG, \frac{1}{|D_\goal|})}{\delta} }{|D_\goal|}} + \sqrt{\epsilon_{\FF,\GG}}  \right)
% \end{align*}
% \end{lemma}
% \begin{proof}
% This follows from Theorem 8 of \citep{cheng2022adversarially}. $\ell_\goal (\bar{f}_g) = 0$ because the reward $R(x)$ is deterministic.
% \end{proof}
\begin{lemma}\label{lm:Qpi in the set}
With probability at least $1-\delta$, it holds for all $\pi\in\Pi$,
\begin{align*}
        &\ell_\dyn( \bar{Q}^{\bar{\pi}},  \bar{Q}^{\bar{\pi}} ;\bar\pi) - \min_{\bar{f}_{g'}'\in\bar\FF} \ell_\dyn(\bar{f}_{g'}', \bar{Q}^{\bar{\pi}} ;\bar\pi) \leq \epsilon_\dyn\\
    &\ell_\goal (\bar{Q}^{\bar{\pi}}) \leq 0 
\end{align*}
%\aditya{Is $\tilde f^\pi_g$ supposed to be $\bar f_R$?}
%where $\bar{Q}_R^\pi $ denotes the extension of $\bar{Q}^\pi$ based on $R$, and
where\footnote{Technically, we can remove $ \NN_\infty(\GG, \frac{1}{|D_\dyn|}) $ in the upper bound, but including it make the presentation cleaner.}
\begin{align*}
    &\epsilon_\dyn = O\left( {\frac{\log \frac{ \NN_\infty\left(\FF, \frac{1}{|D_\dyn|}\right) \NN_\infty\left(\GG, \frac{1}{|D_\dyn|}\right) \NN_{\infty,1}\left(\Pi,\frac{1}{|D_\dyn|}\right)}{\delta} }{|D_\dyn|}}  \right)
    % &\epsilon_\goal = O\left( \sqrt{\frac{\log \frac{\NN_\infty(\GG, \frac{1}{|D_\goal|})}{\delta} }{|D_\goal|}} + \sqrt{\epsilon_{\FF,\GG}}  \right)
\end{align*}
\end{lemma}
\begin{proof}
% \chingan{Updated}
%Note that $\bar{Q}^{\bar\pi} = \bar{Q}_R^{\pi}$ on the support of $\mu_\dyn$ and 
Note $\bar{Q}^{\bar\pi} = \bar{f}_g$ for some $f\in\FF$ and $g\in\GG$ (\cref{lm:realizability}) and 
\begin{align*}
 0 = \E_{x,a\sim\mu_\dyn} [(\bar{Q}^{\bar\pi}(x,a) - \bar\TT^{\bar\pi} \bar{Q}^{\bar\pi}(x,a))^2] 
 &= 
 \E_{x,a\sim\mu_\dyn} [(\bar{Q}^{\bar\pi}(x,a) - 0 - \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [ \phi(\bar{Q}^{\bar\pi})(x',\pi) ] )^2]
\end{align*}
Following a similar proof of Theorem 8 of \citep{cheng2022adversarially}, we can derive $\epsilon_\dyn$. On the other hand, $\ell_\goal (\bar{f}_g) = 0$ because the reward $R(x)$ is deterministic.
\end{proof}



Nest, we show that with high probability the empirical error can upper bound the population error.
\begin{lemma}\label{lm:generalization error)}
For all $f\in\FF,g\in\GG$ satisfying 
\begin{align*}
        &\ell_\dyn( \bar{f}_g, \bar{f}_g ;\bar\pi) - \min_{\bar{f}_{g'}'\in\bar\FF} \ell_\dyn(\bar{f}_{g'}',\bar{f}_g;\bar\pi) \leq \epsilon_\dyn \\
    &\ell_\goal (\bar{f}_g) \leq  0
\end{align*}
With probability at least $1-\delta$, for any $f\in\FF$,$g\in\GG$
\begin{align*}
    &\left\| \bar{f}_g(x,a) - \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [\max(g(x'), f(x',\pi))] \right\|_{\mu_\dyn}
    \leq O\left( \sqrt{\epsilon_\dyn} \right) \\
    %+ \sqrt{\frac{\log \frac{ \NN_\infty(\FF, \frac{1}{|D_\dyn|})\NN_\infty(\GG, \frac{1}{|D_\dyn|}) \NN_{\infty,1}(\Pi,\frac{1}{|D_\dyn|})}{\delta} }{|D_\dyn|}} \right)\\
        % &L_\dyn( \bar{f}_g, \bar{f}_g ;\bar\pi)  \leq \epsilon_b + \epsilon'\\
    % &L (\bar{f}_g) \leq \epsilon_b + \epsilon'
    %
    &\left\| g(x) - 1\right\|_{\mu_\goal}
    \leq O\left(   \sqrt{\frac{\log \frac{ \NN_\infty\left(\GG, \frac{1}{|D_\goal|}\right)}{\delta} }{|D_\goal|}} \right) \eqcolon \sqrt{\epsilon_\goal}
\end{align*}
\end{lemma}
\begin{proof}
This follows from Theorem 9 of \citep{cheng2022adversarially}. 
\end{proof}


% Suppose $\epsilon_b$ is chosen correctly such that the following is true.
% \begin{align*}
%         &\ell_\dyn( \bar{f}_g, \bar{f}_g ;\bar\pi) - \min_{\bar{f}_{g'}'\in\bar\FF} \ell_\dyn(\bar{f}_{g'}',\bar{f}_g;\bar\pi) \leq \epsilon_b\\
%     &\ell_\goal (\bar{f}_g) \leq \epsilon_b
% \end{align*}
% would imply 
% \begin{align*}
%     &\E_{\mu_\dyn} ( f(x,a) - \gamma \E_{x'\sim \bar{P}(\cdot|x,a)} [   \max(g(x'), f(x', \pi))  ]   )^2 \leq \epsilon_b \\
%     &\E_{\mu_\goal}  ( g(x) -1   )^2 \leq \epsilon_b
% \end{align*}
% We denote this set on $\FF$ on $\GG$ as $\Omega_\stat$



\paragraph{Pessimistic Estimate}

We show the empirical value estimate found in \eqref{eq:pspi (augemnted) (real)} is pessimistic.
\begin{lemma}
Given $\pi$, let $\bar{f}_g^{\pi}$ denote the minimizer in \eqref{eq:pspi (augemnted) (real)}. 
With high probability, 
    $\bar{f}_g^\pi (d_0, \bar\pi) \leq Q^{\pi}(d_0, \pi) $%\sqrt{\epsilon_{\FF,\GG}}$
\end{lemma}
\begin{proof}
    By \cref{lm:Qpi in the set}, we have 
    $\bar{f}_g^\pi (d_0, \bar\pi) \leq \bar{Q}_R^{\pi}(d_0, \bar\pi) = Q^{\pi}(d_0, \pi) $.
\end{proof}
% \begin{proof}
%     \begin{align*}
%         &\bar{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) \\
%         &= \bar{f}_g^\pi (d_0, \bar\pi) - \tilde{f}_g^\pi (d_0, \bar\pi) + \tilde{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) \\        
%         &\leq \tilde{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) 
%     \end{align*}
%     where the inequality is due to that $\bar{f}_g^{\pi}$ is the minimizer in \eqref{eq:pspi (augemnted) (real)}. 
%     %
%     We can expand the last term as 
%     % \begin{align*}
%     %      &\tilde{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}_g^\pi (x_t, \bar\pi) - R(x_t) - \gamma \tilde{f}_g^\pi (x_{t+1},\bar\pi)) + \gamma^T (\tilde{f}_g^\pi (x_{T},\bar\pi) - R(x_T))  \right] \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \tilde{f}_g^\pi(x_{t+1}, \bar{\pi})) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \max(R(x_{t+1}), \tilde{f}_g^\pi(x_{t+1}, \pi))) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     
%     % \end{align*}

%     % \begin{align*}
%     %      &\tilde{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-2} \gamma^t (\tilde{f}_g^\pi (x_t, \bar\pi) - R(x_t) - \gamma \tilde{f}_g^\pi (x_{t+1},\bar\pi)) + \gamma^{T-1} (\tilde{f}_g^\pi (x_{T-1},\bar\pi) - R(x_{T-1}) - \gamma R(x_T) )  \right] \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-2} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \tilde{f}_g^\pi(x_{t+1}, \bar{\pi})) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     \\
%     %     &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \max(R(x_{t+1}), \tilde{f}_g^\pi(x_{t+1}, \pi))) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     
%     % \end{align*}
    
%     % For $t<T-1$
%     % \begin{align*}
%     %     - \max(R(x_{t+1}), \tilde{f}^\pi(x_{t+1}, \pi))
%     %     &= - \max(R(x_{t+1}), \tilde{f}^\pi(x_{t+1}, \pi)) \\
%     %     &\leq - \max(\tilde{g}^\pi(x_{t+1}), \tilde{f}^\pi(x_{t+1}, \pi)) + | R(x_{t+1}) - \tilde{g}^\pi(x_{t+1})|\\
%     % \end{align*}
%     % For $t=T-1$, 

%      \begin{align*}
%          &\tilde{f}_g^\pi (d_0, \bar\pi) - Q^{\pi}(d_0, \pi) \\
%         &= \tilde{f}^\pi (d_0, \pi) - Q^{\pi}(d_0, \pi) \\
%         &\leq \frac{1}{1-\gamma} \epsilon_{\FF,\GG}
%         % &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,\pi) - R(x_t) - \gamma \tilde{f}^\pi (x_{t+1},\pi)) + \gamma^T (\tilde{f}^\pi (x_{T},\pi) - R(x_T))  \right] \\
%         % &= \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \tilde{f}_g^\pi(x_{t+1}, {\pi})) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     \\
%         % &\leq \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t (\tilde{f}^\pi (x_t,a)  - \gamma \max(g(x_{t+1}, \tilde{f}^\pi(x_{t+1}, \pi))) + \gamma^T (\tilde{g}^\pi (x_{T}) - 1  )\right]     
%     \end{align*}
% \end{proof}

% \begin{align*}
%     &(1-\gamma) Q^\pi(s_0, \pi) \\
%     & = (1-\gamma) Q^\pi(s_0, \pi) + \frac{\beta}{2} \left( \E_\mu \left(  \bar{R}(x) + \mathbb{E}_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))] - Q^{\pi}(x,a)   \right)^2 +  \E_\rho (R(x') - R(x'))^2 \right)\\
%     &= \min_{f,g} (1-\gamma) f(s_0, \pi) + \frac{\beta}{2} \left( \E_\mu \left(  g(x) + \mathbb{E}_{x'\sim \bar{P}(\cdot|x,a)} [   \max(g(x'), f(x', \pi))] - f(x,a)   \right)^2 + \E_\rho (g(x') - R(x'))^2 \right)\\
%     &\geq f^\pi(s_0, \pi)
% \end{align*}
% % \aditya{Should be $\bar{R}(x) \textcolor{red}{+} \mathbb{E}_{x'\sim \bar{P}(\cdot|x,a)} [   \max(R(x'),Q^{\pi}(x', \pi))] - Q^{\pi}(x,a)$}

Next we bound the amount of underestimation.
\begin{lemma}
Suppose $x_0\sim d_0$ is not in $G$ almost surely. For any $\pi\in\Pi$,
%
\begin{align*}
    &Q^\pi(d_0, \pi) - \bar{f}_g^\pi(d_0, \bar\pi) \\
    &\leq \E_{\pi} \left[ \sum_{t=0}^{T-1} \gamma^{t}  \left( \gamma \max(g^\pi(x_{t+1}), f^\pi(x_{t+1}, \pi)) - f^\pi(x_t,a_t)\right)  + \gamma^T ( R(x_T) - g^\pi(x_T) )\right]
\end{align*}
Note that in a trajectory $x_T\in G$ whereas $x_t\notin G$ for $t<T$ by definition of $T$.
\end{lemma}


\begin{proof}
Let $\bar{f}_g^{\pi} = (f^\pi, g^\pi)$ be the empirical minimizer.
By performance difference lemma, we can write %\aditya{Should be $x_0$ throughout instead of $d_0$?}
\begin{align*}
    % &(1-\gamma) Q^\pi(x_0, \pi) - (1-\gamma) f^\pi(x_0, \pi) \\
    &(1-\gamma) Q^\pi(d_0, \pi)  - (1-\gamma) \bar{f}_g^\pi(d_0, \bar{\pi}) \\
    &= (1-\gamma) \bar{Q}^\pi(d_0, \bar{\pi}) - (1-\gamma)\bar{f}_g^\pi(d_0, \bar{\pi}) \\
    &= \E_{\bar{d}^{\bar\pi}}[ \bar{R}(x,a) + \gamma \bar{f}_g^\pi(x',\bar{\pi}) - \bar{f}_g^\pi(x,a)]
\end{align*}
where with abuse of notation we define $\bar{d}^{\bar\pi}(x,a,x') \coloneq \bar{d}^{\bar\pi}(x,a) \bar{P}(x'|x,a)$, where $\bar{d}^{\bar\pi}(x,a)$ is the average state-action distribution of $\bar{\pi}$ in the augmented MDP.

In the above expectation, for $x\in G$, we have $a=a^+$ and $x^+ = (s^+, c)$ after taking $a^+$ at $x = (s,c)$, which leads to 
\begin{align*}
     \bar{R}(x,a) + \gamma \bar{f}_g^\pi(x',\bar{\pi}) - \bar{f}_g^\pi(x,a)
    = \bar{R}(x,a^+) + \gamma \bar{f}_g^\pi(x^+,\bar{\pi}) - \bar{f}_g^\pi(x,a^+)
    = R(x) - g^\pi(x)
\end{align*}
For $x\notin G$ and $x\notin\XX^+$, we have $a\neq a^+$ and $x'\notin \XX^+$; therefore
\begin{align*}
    \bar{R}(x,a) + \gamma \bar{f}_g^\pi(x',\bar{\pi}) - \bar{f}_g^\pi(x,a)
    &= R(x) + \gamma \bar{f}_g^\pi(x',\bar{\pi}) - f^\pi(x,a)\\
    &\leq \gamma \max(g^\pi(x'), f^\pi(x',\pi)) - f^\pi(x,a)
\end{align*}
where the last step is because of the definition of $\bar{f}_g^\pi$.
For $x\in\XX^+$, we have $x\in\XX^+$ and the reward is zero, so 
\begin{align*}
    \bar{R}(x,a) + \gamma \bar{f}_g^\pi(x',\bar{\pi}) - \bar{f}_g^\pi(x,a)
    = 0 
\end{align*}


Therefore, we can derive
\begin{align*}
    &(1-\gamma) Q^\pi(x_0, \pi) - (1-\gamma) \bar{f}_g^\pi(x_0, \bar\pi) \\
    &\leq \E_{\bar{d}^{\bar\pi}}[     \gamma \max(g^\pi(x'), f^\pi(x',\pi)) - f^\pi(x,a)  | x \notin G, x\notin \XX^+ ]
    + \E_{\bar{d}^{\bar\pi}}[ R(x) - g^\pi(x) | x\in G]
\end{align*}
Finally, using \cref{lm:equivalence} we can have the final upper bound.


\end{proof}


\subsection{Main Result: Performance Bound}

Let $\pi^\dagger$ be the learned policy and let $\bar{f}_g^{\pi^\dagger}$ be the learned function approximators. 
For any comparator policy $\pi$, let $\bar{f}_g^\pi = (f^\pi,g^\pi)$ be the estimator of $\pi$ on the data. We have.
\begin{align*}
&  V^\pi(d_0) - V^{\pi^\dagger}(d_0)\\
&=  Q^\pi(d_0, \pi) - Q^{\pi^\dagger}(d_0, \pi^\dagger) \\
&=  Q^\pi(d_0, \pi) - \bar{f}_g^{\pi^\dagger}(d_0, \bar{\pi}^\dagger) + \bar{f}_g^{\pi^\dagger}(d_0, \bar{\pi}^\dagger) - Q^{\pi^\dagger}(d_0, \pi^\dagger) \\
&\leq Q^\pi(d_0, \pi) - \bar{f}_g^{\pi^\dagger}(d_0, \bar{\pi}^\dagger)\\
&\leq Q^\pi(d_0, \pi) - \bar{f}_g^{\pi}(d_0, \bar{\pi})\\
&\leq \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t ( \gamma \max(g^\pi(x_{t+1}), f^\pi(x_{t+1}, \pi)) - f^\pi(x_t,a_t)) + \gamma^T (  R(x_T) - g^\pi(x_T)) \right]\\
&\leq \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t |\gamma \max(g^\pi(x_{t+1}), f^\pi(x_{t+1}, \pi)) - f^\pi(x_t,a_t)|  + \gamma^T | R(x_T) - g^\pi(x_T)| \right]\\
&\leq \mathfrak{C}_\dyn(\pi) \E_{\mu_\dyn}[ |\gamma \max(g^\pi(x'), f^\pi(x', \pi)) - f^\pi(x,a)|]
+  \mathfrak{C}_\goal(\pi) \E_{\mu_\goal}[ |g(x) - 1|]\\
&\leq  \mathfrak{C}_\dyn(\pi) \sqrt{\epsilon_\dyn} + 
    +  \mathfrak{C}_\goal(\pi) \sqrt{\epsilon_\goal}
\end{align*}
where 
\begin{align*}
    \mathfrak{C}_\dyn(\pi) = \mathfrak{C}_\dyn( \rho_{\notin G}^\pi, \mu_\dyn, \FF, \pi) \\
    \mathfrak{C}_\goal(\pi) = \mathfrak{C}_\dyn( \rho_{\in G}^\pi, \mu_\goal, \GG, \pi) 
\end{align*}
and 
\begin{align*}
    \rho_{\notin G}^\pi(x,a) &= 
    \E_{\pi,P} \left[ \sum_{t=0}^{T-1} \gamma^t \one(x_t=x, a_t=a)  \right]\\
    \rho_{\in G}^\pi(x) &= 
    \E_{\pi,P} \left[ \gamma^T \one(x_T=x)  \right]\\
\end{align*}

\begin{theorem}
    Let $\pi^\dagger$ denote the learned policy. Under the above assumptions, with high probability, it holds, for any $\pi\in\Pi$,
    \begin{align*}
    V^\pi(d_0) - V^{\pi^\dagger}(d_0)
    &\leq  \mathfrak{C}_\dyn(\pi) \sqrt{\epsilon_\dyn} 
    +  \mathfrak{C}_\goal(\pi) \sqrt{\epsilon_\goal}
    \end{align*}
\end{theorem}
% \chingan{Need to double check the notations.}


% For $x_0 \notin G$,
% \begin{align*}
%     &(1-\gamma) Q^\pi(x_0, \pi) - (1-\gamma) f^\pi(x_0, \pi) \\
%     &= (1-\gamma) \bar{Q}^{\bar{\pi}}(d_0, \bar{\pi}) - (1-\gamma) \bar{f}^\pi(x_0, \bar{\pi}) \\
%     &= \E_{\bar{d}_{x_0}^{\bar\pi}}[ \bar{R}(x,a) + \gamma \bar{f}^\pi(x',\bar{\pi}) - \bar{f}^\pi(x,a)]
% \end{align*}
% where $\bar{d}_{x_0}^{\bar\pi}$ denotes the discounted average state-action distribution/occupancy meaure of the augmented MDP. 

% For $x\in G$, we have
% \begin{align*}
%     \E_{\bar\pi}[  \bar{R}(x,a) + \gamma \bar{f}^\pi(x',\bar{\pi}) - \bar{f}^\pi(x,a)]
%     = \bar{R}(x,a^+) + \gamma \bar{f}^\pi(x^+,\bar{\pi}) - \bar{f}^\pi(x,a^+)
%     = R(x) - g^\pi(x)
% \end{align*}

% For $x\notin G$, we have
% \begin{align*}
%     \E_{\bar\pi}[  \bar{R}(x,a) + \gamma \bar{f}^\pi(x',\bar{\pi}) - \bar{f}^\pi(x,a)]
%     &= \E_{\bar\pi}[  R(x) + \gamma \bar{f}^\pi(x',\bar{\pi}) - f^\pi(x,a)]\\
%     &\leq \E_{\bar\pi}[  R(x) + \gamma \max(g^\pi(x'), f^\pi(x',\pi)) - f^\pi(x,a)]
% \end{align*}
% where the last step is because of the definition of $\bar{f}^\pi$.
% Therefore, we can write 
% \begin{align*}
%     &(1-\gamma) Q^\pi(x_0, \pi) - (1-\gamma) f^\pi(x_0, \pi) \\
%     &= \E_{\bar{d}_{x_0}^{\bar\pi}}[     R(x) + \gamma \max(g^\pi(x'), f^\pi(x',\pi)) - f^\pi(x,a)  | x \notin G]
%     + \E_{\bar{d}_{x_0}^{\bar\pi}}[ R(x) - g^\pi(x) | x\in G]
% \end{align*}
% We can bound these two terms with the training error.
% \chingan{TODO: rewrite the expectation back to $d^\pi$. Maybe we don't need to move the augmented MDP to begin with in this expansion.}


